Two Structural Results for Low Degree Polynomials and Applications

In this paper, two structural results concerning low degree polynomials over finite fields are given. The first states that over any finite field $\mathbb{F}$, for any polynomial $f$ on $n$ variables with degree $d \le \log(n)/10$, there exists a subspace of $\mathbb{F}^n$ with dimension $\Omega(d \cdot n^{1/(d-1)})$ on which $f$ is constant. This result is shown to be tight. Stated differently, a degree $d$ polynomial cannot compute an affine disperser for dimension smaller than $\Omega(d \cdot n^{1/(d-1)})$. Using a recursive argument, we obtain our second structural result, showing that any degree $d$ polynomial $f$ induces a partition of $F^n$ to affine subspaces of dimension $\Omega(n^{1/(d-1)!})$, such that $f$ is constant on each part. We extend both structural results to more than one polynomial. We further prove an analog of the first structural result to sparse polynomials (with no restriction on the degree) and to functions that are close to low degree polynomials. We also consider the algorithmic aspect of the two structural results. Our structural results have various applications, two of which are: * Dvir [CC 2012] introduced the notion of extractors for varieties, and gave explicit constructions of such extractors over large fields. We show that over any finite field, any affine extractor is also an extractor for varieties with related parameters. Our reduction also holds for dispersers, and we conclude that Shaltiel's affine disperser [FOCS 2011] is a disperser for varieties over $F_2$. * Ben-Sasson and Kopparty [SIAM J. C 2012] proved that any degree 3 affine disperser over a prime field is also an affine extractor with related parameters. Using our structural results, and based on the work of Kaufman and Lovett [FOCS 2008] and Haramaty and Shpilka [STOC 2010], we generalize this result to any constant degree.

==> average_case.tex <==
\section{Affine Extractors are Hard to Approximate by Low Degree Polynomials}
\begin{corollary}\label{cor:average_case}
Let $f \colon \B^n \to \B$ be an affine extractor for dimension $k$ with bias $\eps$.
Then, for any polynomial $g$ with degree $d$ such that $k < \Kpart$, it holds that  $\mathrm{Cor}(f, g) < \eps$.
\end{corollary}


\begin{proof}[Proof of Corollary~\ref{cor:average_case}]
Let $g$ be the best approximation of $f$ among all polynomials of degree $\le d$.
By Theorem~\ref{thm:partition to constants}, there exists a partition of $\F_2^n$ to affine subspaces $P_1, P_2,
\ldots, P_\ell$, each of dimension $\Kpart$, such that the $g|_{P_i}$ is constant for all $i\in[\ell]$.
%Since $g$ is an affine extractor for dimension $k < \Kpart$ with bias $\eps$ then $\bias(g \oplus f) \le \eps$. By averaging,
\[
\mathrm{Cor}(f,g) =
\left|\E_{x \sim \F_2^n}[(-1)^{f(x)+g(x)}]\right| =
\left|\E_{i\sim[\ell]} \E_{x\sim P_i} [(-1)^{f(x)+g(x)}]\right| \le
\E_{i\sim[\ell]} \left|\E_{x\sim P_i} [(-1)^{f(x)+g(x)}]\right| \le \eps,
\]
where the last inequality follows since $f$ is an affine extractor for dimension $k < \Kpart$ with bias $\eps$.
\end{proof}


==> structal_extra.tex <==
\begin{theorem}[Structural Result II for many polynomials]\label{thm:structural result II for many polynomials}
There exists a constant $\alpha'$ such that the following holds. Let $f_1, \ldots, f_t$ be polynomials in $n$ variables over $\F_2$, each of degree at most $d$. Then, there exists a partition of $\F_2^n$ to affine subspaces, each of dimension $\alpha' \cdot \frac{n^{1/(d-1)!} }{t^{e}} - d$, such that $f_1,\ldots,f_t$ are all constant on each part.
\end{theorem}

\begin{proof}

Let $\alpha$ be the constant from Theorem~\ref{thm:structural result}. Define the sequence $\{\beta_d \}_{d=1}^{\infty}$ as follows.
$$
\beta_d =
\left\{
  \begin{array}{ll}
    1, & \hbox{$d=1$} \\
    \beta_{d-1} \cdot \alpha^{\frac1{(d-2)!}}, & \hbox{$1 < d$}
  \end{array}
\right.
$$
We will prove by induction on $d$, the degree of a given polynomial $f$, that there exists a partition of $\F_2^n$ to affine subspaces of dimension $\ge \beta_d \cdot \frac{n^{1/(d-1)!}}{t^{1/1!+\ldots+1/(d-1)!}} - d - t$, such that $f$ restricted to each part is constant. 
The base case of the induction, namely $d=1$, trivially follows as $f_1, \ldots, f_t$ are affine functions, and we can partition $\F_2^n$ to affine subspaces of dimension $n-t$ on which $f_1, \ldots, f_t$ are constant.

Assume now that $d > 1$. There exists a partition of $\F_2^n$ to affine subspaces of dimension $k \ge \max\{\Ksubspacevar,0\}$, such that $f_1, \ldots, f_t$ restricted to any affine subspace in the partition has degree at most $d-1$.

Fix some affine subspace $u_0 + U$ in the partition and apply the induction hypothesis to the polynomials $f_i' = f_i|_{u_0 + U}$, which has degree $\le d-1$. We note that we may apply the induction because there exists a linear bijection from $U$ to $\F_2^{\dim{U}}$. More precisely, if $A$ is an $n \times k$ matrix over $\F_2$ that maps $U$ to $\F_2^k$ bijectively, then one can apply the induction to the polynomial $f_i''(x) = f_i'(u_0 + Ax)$, defined on $k$ variables, and then induce a partition of $u_0 + U$ from the partition of $\F_2^k$ obtained by the induction. The induction can be carried on $f_i''$ since $d_i'' := \deg{f_i''} \le \deg{f_i'} \le d-1$, where the first inequality holds because the variables of $f_i''$ are linear combinations of the variables of $f_i'$.

By the induction hypothesis, we obtain a partition of $u_0 + U$ such that, on each part, $f_i$ are constant. Moreover, the dimension of each such part is at least
\begin{align*}
\beta_{d-1} \cdot \frac{k^{\frac1{(d-2)!}}}{t^{1/1!+\ldots+1/(d-2)!}} - (d-1) - t \\
&=   \beta_{d-1} \cdot \frac{\left( \max\{\Ksubspacevar,0\} \right)^{\frac1{(d-2)!}}}{t^{1/1!+\ldots+1/(d-2)!}}  - (d-1) -t\\
&\ge \beta_{d-1} \cdot \frac{\left(\left( \alpha \cdot (n/t)^{\frac1{d-1}} \right)^{\frac1{(d-2)!}} - 1\right)}{t^{1/1!+\ldots+1/(d-2)!}} - (d-1) -t \\
&\ge \beta_{d-1} \cdot \alpha^{1/(d-2)!} \cdot \frac{n^{\frac1{(d-1)!}}}{t^{1/1!+\ldots+1/(d-1)!}} - d - t\\
& = \beta_d \cdot \frac{n^{\frac1{(d-1)!}}}{t^{1/1!+\ldots+1/(d-1)!}} - d - t\;,
\end{align*}
where the first inequality follows since $(\max\{x-1,0\})^{1/(d-2)!} \ge x^{1/(d-2)!} -1$ for any $x \ge 0$; and the last follows since $\frac{\beta_{d-1}}{t^{1/1!+\ldots+1/(d-2)!}} \le 1$.
\end{proof}

==> structural_Fp.tex <==
\section{Structural Result over $\F_p$}
Let $f \in \F_p [x_1, \ldots, x_n]$ be a polynomial of degree $d$, and such that each individual degree is at most $p-1$.
For $\alpha \in \F_p^n$ we denote by $|\alpha| = \sum_{i=1}^{n}{\alpha_i}$ where the sum is over the integers.
\begin{fact}
Let $f$ be a polynomial of degree $d$ then
$\frac{\partial f}{\partial{\Delta}} (x) \deff f(x+\Delta) - f(x)$ is a polynomial of degree $\le d- 1$.
\end{fact}


%\begin{claim}
%Let $f = \sum_{\beta} c_\beta \prod_{i=1}^{n} {x_i^{\beta_i}}$ of degree $d$ then
%$\frac{\partial f}{\partial^{\alpha_1} {e_1} \cdots \partial^{\alpha_n} {e_n}} \equiv
%c_{\alpha}$  for any $\alpha$ of weight $d$.
%\end{claim}
%\begin{proof}
%It is enough to show this when $f$ is a monomial of total degree at most $d$ as derivatives are linear operators.
%So assume $f = \prod_{i=1}^{n}{x_i^{\beta_i}}$.
%If $\beta_i < \alpha_i$ for some $i$ then $\frac{\partial{f}}{\partial^{\alpha_i}(e_i)} = 0$.
%So we assume all $\beta_i \ge \alpha_i$, which implies that $\alpha=\beta$ (since if there is a coordinate in which $\beta_i > \alpha_i$ then the total degree of $\beta$ is at least $d+1$). For $\alpha=\beta$ we get that $\frac{\partial{x_i^{\alpha_i}}}{\partial^{\alpha_i}(e_i)} = 1$ and we deduce this for general monomials.
%\end{proof}

\begin{claim}\label{claim:derivatives_is_enough}
$f \equiv 0$ iff $\frac{\partial{f}}{\partial^{\alpha_1}(e_1) \ldots \partial^{\alpha_n}(e_n)}(0) = 0$ for all $\alpha \in \F_p^n$.
\end{claim}
\begin{proof}
If $f \equiv 0$ this is obvious.
Assume not, then take some maximal monomial in $f$'s representation as a polynomial with each variable having degree $\le p-1$, Applying the derivative with $\alpha$ makes all other monomials zero and this monomial is $1$.
\end{proof}
\begin{corollary}\label{cor:derivatives_is_enough}
Let $U = \spa\{\Delta_1, \ldots, \Delta_k\}$ a subspace of $\F_p^n$ and $x\in\F_p^n$, then
$f|_{x + U}  \equiv 0$ iff $\frac{\partial{f}}{\partial^{\alpha_1}(\Delta_1) \ldots \partial^{\alpha_k}(\Delta_k)}(x) = 0$ for all $\alpha \in \F_p^k$.
\end{corollary}

In particular given a polynomial of degree at most $d$ it is enough to check if it the all zero polynomial by checking if all its derivatives up to weight $d$ are zero. This is a local test which only observes the polynomial value on vectors of hamming weight at most $d$.

Adaptation of the proof for $\F_2$ into general $\F_p$:

\begin{theorem}[Structural Result I]\label{thm:structural result Fp}
Let $k$ be the smallest integer such that
\[
n \le k + d \cdot \sum_{j=0}^{d-1} {(d-j) \cdot \binom{k+j-1}{j}}\;.
\]
Let $f \colon \F_p^n \to \F_p$ be a degree $d$ polynomial, and let $u_0 \in \F_p^n$. Then, there exists a subspace $U \subset \F_p^n$ of dimension $k$ such that $f|_{u_0+U}$ is constant.
\end{theorem}

The Theorem implies that $n \le (1+d^2) \cdot \binom{k + d-1}{d-1}$, which means that $k + d-1 \ge 1/28 d n^{1/(d-1)}$.
For $d \le 1/10 \log n$ we get $k = \Omega(d \cdot n^{1/(d-1)})$.

Upper bound:
A random polynomial is constant on an affine subspace of dimension $k$ with probability $p^{-\binom{k + d}{d}}$
\footnote{This is not totally accurate since the number of monomials could be less than $\binom{k+d}{d}$ if $d>p$. To be precise $\binom{k+d}{d}$ should be replaced by the number of solutions to the equation $r_1 + \ldots + r_k \le d$ where $r_i \in \{0,\ldots, p-1\}$.}
 There are at most $p^{(k+1)n}$ affine subspaces of dimension $k$ so overall we get that if $\binom{k+d}{d} > (k+1)n$ then there exists a polynomial of degree $d$ which is an affine disperser for dimension $k$.
The ratio between the two upper and lower bounds is roughly $d^{1/d}$.

The proof of Theorem \ref{thm:structural result Fp} uses a folklore variant of the Schwartz-Zippel lemma for small fields.

\begin{claim}\label{claim:schwartz Fp}
Let $f \colon \F_p^n \to \F_p$ be a non-zero degree $d$ polynomial. Then,
\[
\Pr_{x \sim \F_p^n}[f(x) \neq 0] \ge p^{-d/(p-1)}.
\]
\end{claim}

\begin{proof}[Proof of Theorem \ref{thm:structural result Fp}]
%The claim is true for $d=1$ (with $\alpha =1$), so we may assume for the rest of the proof that $d \ge 2$.
Fix $u_0\in \F_p^n$.
We assume without loss of generality that $f(u_0) = 0$, as otherwise we can look at the polynomial $g(x) = f(x)-f(u_0)$ which is of the same degree.
The proof is by induction.
Let $k$ be such that
\begin{equation}\label{eq:condition on k}
n > k + d \cdot \sum_{j=0}^{d-1} {(d-j) \cdot \binom{k+j-1}{j}} \;.
\end{equation}
We assume by induction that there exists an affine subspace $u_0 + \spa\{\Delta_1, \ldots, \Delta_k\} \subseteq \F_p^n$, where the $\Delta_i$'s are linearly independent vectors on which $f$ evaluates to 0.
Assuming Equation~\ref{eq:condition on k} holds, we show there exists a vector $\Delta_{k+1}$, linearly independent of $\Delta_1, \ldots, \Delta_k$, such that $f \equiv 0$ on $u_0 + \spa\{\Delta_1, \ldots, \Delta_{k+1}\}$. To this aim, consider the set
\[
A = \left\{
x\in \F_p^n\;\;\; \bigg\vert\;\;\; \forall{\alpha \in \F_p^k},\;{f\(x + \sum_{i} {\alpha_i \Delta_i}\) = 0}
\right\}.
\]
By the induction hypothesis, $u_0 \in A$. Using Corollary~\ref{cor:derivatives_is_enough} we get that for any $x \in \F_p^n$,
\[
\forall{\alpha\in \F_p^k}: f\(x + \sum_{i} {\alpha_i \Delta_i}\) = 0 \quad \Leftrightarrow \quad
\forall{\alpha}: f_\alpha(x) = 0 \;,
\]
where $f_\alpha$ is defined by
\[
f_\alpha(x) \deff \frac{\partial{f}}{\partial^{\alpha_1}(\Delta_1) \ldots \partial^{\alpha_k}(\Delta_k)} (x).
\]
In particular, $\deg(f_\alpha) \le d-|\alpha|$. Thus $f_\alpha \equiv 0$ for $|\alpha| > d$, and we may write $A$ as
\[
A = \left\{
x \in \F_p^n \;\mid\; \forall{\alpha:|\alpha|\le d} ,\; f_\alpha(x) = 0
\right\}.
\]
Hence, $A$ is the set of solutions to a system of $\le \binom{k+d}{d}$ polynomial equations,
where there are $\binom{k+j-1}{j}$ equations which correspond to $\alpha$'s of weight $j$ and thus to degree (at most) $d-j$ polynomials.
One can also write $A$ as the set of non-zeros to the single polynomial
\[
t(x) := \prod_{\alpha:|\alpha|\le d}{\!\!\!\!\!\! (1-f_\alpha(x)^{p-1})} \,\,,
\]
which is of degree
\[
\deg(t) \le (p-1) \cdot \sum_{j=0}^{d-1} {(d-j) \cdot \binom{k+j-1}{j}}\;.
\]

Now we wish to find a new direction $\Delta_{k+1}$. We want
\begin{equation}\label{eq:condition_on_delta}
1 = t(u_0 + i\Delta_{k+1})  \text{~for~} i=0,\ldots, \min\{d,p-1\}
\end{equation}
 This will imply that $f$ equals $0$ on the Hamming ball of radius $d$ around $u_0$ with respect to the basis $\Delta_1, \ldots, \Delta_{k+1}$, which implies that $f|_{u_0 + \spa\{\Delta_1, \ldots, \Delta_{k+1}\}} \equiv 0$.
View the set of Equations~\ref{eq:condition_on_delta} as equations on $\Delta_{k+1}$.
Define a polynomial
\[
s(y) := \prod_{i=0}^{\min\{d,p-1\}} t(u_0 + i \cdot y)
\]
The non-zeros of $s(y)$ are exactly all possible directions $\Delta_{k+1}$ such that all points on the line $\{u_0 + i\Delta_{k+1}\}_{i=0,\ldots, \min\{d,p-1\}}$ are in the set $A$. The question remains, does there exists such $\Delta_{k+1}$ which is linearly dependent of $\{\Delta_1, \ldots \Delta_{k}\}$.
Since the trivial solution $y = 0$ is a non-zero for $s$, this means that we can apply Claim~\ref{claim:schwartz Fp}.
We get that there exist at least $p^{n-\deg(s)/(p-1)}$ possible solutions. Since we need to avoid $p^{k}$ linear combinations of the previous $\Delta_1, \ldots, \Delta_{k}$ it is enough to show that
$$ n - \frac{\deg(s)}{q-1} > k\;.$$
Since $\deg(s) \le d \cdot (p-1) \cdot \sum_{j=0}^{d-1} {(d-j) \cdot \binom{k+j-1}{j}}$ and by the assumption on $k$ in Equation~\eqref{eq:condition on k}, we get $n - \deg(s)/(p-1) > k$ as required.

\end{proof} 
